Revisiting the Resource Curse in the Age of Energy Transition: Cobalt Reserves and Conflict in Africa

This study reevaluates the traditional understanding of the "political resource curse" by examining the unique impact of energy transition metals, specifically cobalt, on local-level conflicts in Africa. Contrary to previous studies that primarily focus on high-value minerals and their political outcomes resulted from substantial economic revenues, this study investigates cobalt's influence on local conflict. Despite its strategic importance, cobalt's limited commercial value presents a unique yet critical case for analysis. Different with the prevailing view that links mineral reserves with increased conflict, this research finds that regions rich in cobalt experience a reduction in conflict. This decrease is attributed to enhanced government security measures, which are implemented independently of the economic benefits derived from cobalt as a commodity. The study utilizes a combination of georeferenced data and a difference-in-difference design to analyze the causal relationship between cobalt deposits and regional conflict. The findings suggest that the presence of cobalt deposits leads to enhanced security interventions by governments, effectively reducing the likelihood of non-governmental actors taking control of these territories. This pattern offers a new perspective on the role of energy transition metals in shaping conflict and governance, highlighting the need to reassess theoretical frameworks related to the political implications of natural resources with the ongoing energy revolution.

==> fig_table/diagram.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/diagram.pdf}
    % \vspace{-7mm}
    \caption{Strategic and Commercial Values: Definitions and Examples}
    \label{fig:diagram}
\end{figure}

==> presentation/aid.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cobalt Deposits and Financial Aid from China}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{l*{3}{c}}
\hline\hline
            Dependent Variable:  &\multicolumn{3}{c}{Official Financial Aid from China} \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
$Cobalt \times Post_{2002}$   &       4.258         &       3.434         &       4.384         \\
            &     (7.225)         &     (7.299)         &     (6.931)         \\
[1em]
Cobalt          &       0.859         &       0.803         &      -1.476         \\
            &     (0.974)         &     (0.983)         &     (2.314)         \\
[1em]
$Post_{2002}$      &       5.304\sym{***}&       5.374\sym{***}&       8.302         \\
            &     (1.311)         &     (1.575)         &     (9.577)         \\
[1em]
Controls  &          No         &          Yes         &         Yes     \\
[1em]
Country FE  &          No         &          No         &         Yes         \\
[1em]
Year FE     &          No         &          No         &         Yes         \\
\hline
\(N\)       &       42952         &       37586         &       37586         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize \begin{minipage}{0.8\linewidth} \smallskip \textbf{Note:} Robust standard errors are clustered at country level. \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).   \end{minipage}}\\
\end{tabular}
}
\end{table}
\label{tab: aid}

==> presentation/co_conflict.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cobalt Reserves and Conflict}
\resizebox{0.45\linewidth}{!}{%
\begin{tabular}{l*{3}{c}}
\hline\hline
Dependent Variable: Conflict            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
$Cobalt \times Post_{2002}$   &      -2.210\sym{**} &      -2.195\sym{**} &      -2.045\sym{**} \\
            &     (0.986)         &     (0.983)         &     (0.915)         \\
[1em]
Cobalt          &       2.017\sym{*}  &       1.942\sym{*}  &       1.559         \\
            &     (1.013)         &     (1.018)         &     (0.973)         \\
[1em]
$Post_{2002}$      &       0.135         &       0.249         &      -0.619         \\
            &     (0.152)         &     (0.193)         &     (1.156)         \\
[1em]
Polity      &                     &    -0.00752         &     0.00434         \\
            &                     &    (0.0143)         &    (0.0238)         \\
[1em]
Log(GDP)     &                     &      -0.126         &      -0.410         \\
            &                     &    (0.0985)         &     (0.280)         \\
[1em]
GDP Growth  &                     &     -0.0503         &     -0.0573         \\
            &                     &    (0.0388)         &    (0.0495)         \\
[1em]
Log(Population)     &                     &       0.226\sym{***}&       2.777         \\
            &                     &    (0.0815)         &     (1.661)         \\
[1em]
Country FE  &          No         &          No         &         Yes         \\
[1em]
Year FE     &          No         &          No         &         Yes         \\
\hline
\(N\)       &       87481         &       73772         &       73772         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize \begin{minipage}{0.8\linewidth} \smallskip \textbf{Note:} Robust standard errors are clustered at country level.  \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).   \end{minipage}}\\
\end{tabular}
}
\end{table}
\label{tab: cobalt_conflict}

==> presentation/coexistence.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Copper Reserve and the Probability for Non-state Actor Overtakes Territory}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{l*{3}{>{\centering\arraybackslash}p{0.2\linewidth}}}
\hline\hline
Model:    &\multicolumn{3}{c}{Logit Regression} \\
            Dependent Variable:  &\multicolumn{3}{c}{Binary: Non-government actor overtakes territory} \\
            \cmidrule(r{1em}){2-4}
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
$Copper \times Post_{2002}$   &      -0.946         &      -1.228\sym{*}  &      -1.032         \\
            &     (0.599)         &     (0.694)         &     (0.812)         \\
[1em]
Copper          &      0.0230         &       0.140         &      -0.375         \\
            &     (0.407)         &     (0.407)         &     (1.070)         \\
[1em]
$Post_{2002}$      &      -0.342         &       0.496\sym{*}  &      0.0479         \\
            &     (0.316)         &     (0.284)         &     (1.506)         \\
[1em]
Controls  &          No         &          Yes         &         Yes     \\
[1em]
Country FE  &          No         &          No         &         Yes         \\
[1em]
Year FE     &          No         &          No         &         Yes         \\
\hline
\(N\)       &       65209         &       54398         &       45191         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize \begin{minipage}{\linewidth} \smallskip \textbf{Note:} Robust standard errors are clustered at country level.  \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).   \end{minipage}}\\
\end{tabular}
}
\end{table}
\label{tab: copper}

==> presentation/foreign.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Foreign Ownership and the Probability for Non-state Actor Overtakes Territory}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{l*{3}{>{\centering\arraybackslash}p{0.2\linewidth}}}
\hline\hline
Model:    &\multicolumn{3}{c}{Logit Regression} \\
            Dependent Variable:  &\multicolumn{3}{c}{Binary: Non-government actor overtakes territory} \\
            \cmidrule(r{1em}){2-4}
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
Foreign Ownership  &       0.793         &       0.425         &       0.317         \\
            &     (0.838)         &     (1.106)         &     (1.155)         \\
[1em]
Controls  &          No         &          Yes         &         Yes     \\
[1em]
Country FE  &          No         &          No         &         Yes         \\
[1em]
Year FE     &          No         &          No         &         Yes         \\
\hline
\(N\)       &       65209         &       54398         &       45191         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize \begin{minipage}{\linewidth} \smallskip \textbf{Note:} Robust standard errors are clustered at country level.  \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).   \end{minipage}}\\
\end{tabular}
}
\end{table}
\label{tab: fdi}

==> presentation/mechanism.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cobalt Reserve, Price and the Likelihood for Non-state Actor Overtakes Territory}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{l*{6}{c}}
\hline\hline
Model:    &\multicolumn{6}{c}{Logit Regression} \\
            Dependent Variable:  &\multicolumn{6}{c}{Binary: Non-government actor overtakes territory} \\
                         \cmidrule(r{1em}){2-7}
             &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
$Cobalt \times Post_{2002}$ &      -2.704\sym{**} &      -2.589\sym{*}  &      -2.360\sym{*}  &                     &                     &                     \\
            &     (1.239)         &     (1.346)         &     (1.375)         &                     &                     &                     \\
[1em]
$Cobalt \times Price_{t-1}$&                     &                     &                     &     -0.0125\sym{**} &    -0.00965\sym{*}  &     -0.0111         \\
            &                     &                     &                     &   (0.00518)         &   (0.00496)         &   (0.00698)         \\
Cobalt          &       0.391         &       0.335         &      -0.567         &       0.646         &       0.380         &      -0.303         \\
            &     (0.654)         &     (0.743)         &     (1.334)         &     (0.631)         &     (0.665)         &     (1.029)         \\
[1em]
$Post_{2002}$      &      -0.354         &       0.481\sym{*}  &      0.0563         &                     &                     &                     \\
            &     (0.314)         &     (0.285)         &     (1.504)         &                     &                     &                     \\
[1em]
$Price_{t-1}$  &                     &                     &                     &    -0.00199         &     0.00219         &     0.00103         \\
            &                     &                     &                     &   (0.00143)         &   (0.00143)         &    (0.0126)         \\
Controls  &          No         &          Yes         &         Yes     &    No         &          Yes         &         Yes    \\
[1em]
Country FE  &          No         &          No         &         Yes         &          No         &          No         &         Yes         \\
[1em]
Year FE     &          No         &          No         &         Yes         &          No         &          No         &         Yes         \\
\hline
\(N\)       &       65209         &       54398         &       45191         &       65209         &       54398         &       45191         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize \begin{minipage}{\linewidth} \smallskip \textbf{Note:} Robust standard errors are clustered at country level. \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).   \end{minipage}}\\
\end{tabular}
}
\end{table}
\label{tab: mechanism}

==> tables/foreign_own.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Foreign Ownership and the Probability for Non-state Actor Overtakes Territory}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{l*{3}{>{\centering\arraybackslash}p{0.2\linewidth}}}
\hline\hline
Model:    &\multicolumn{3}{c}{Logit Regression} \\
            Dependent Variable:  &\multicolumn{3}{c}{Binary: Non-government actor overtakes territory} \\
            \cmidrule(r{1em}){2-4}
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
Foreign Ownership  &       0.793         &       0.425         &       0.317         \\
            &     (0.838)         &     (1.106)         &     (1.155)         \\
[1em]
Controls  &          No         &          Yes         &         Yes     \\
[1em]
Country FE  &          No         &          No         &         Yes         \\
[1em]
Year FE     &          No         &          No         &         Yes         \\
\hline
\(N\)       &       65209         &       54398         &       45191         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize \begin{minipage}{0.7\linewidth} \smallskip \textbf{Note:} Robust standard errors are clustered at country level.  \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).   \end{minipage}}\\
\end{tabular}
}
\end{table}
\label{tab: fdi}

==> tables/implications.tex <==
\begin{table}[t]
\caption{Strategic and Commercial Values: Implications to Conflict} 
\label{tab:implications} 
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{p{2.5cm}p{8cm}cp{1.5cm}c}
\toprule[1.1pt]
Value  & Definition & Government & Rebel Group & Conflict \\
\midrule
Strategic Value & Energy Security, Supply Chain Security and Technological Advancement & 0.2624 & 0.2550 & 0.0061 \\
\bottomrule[1.1pt]
\end{tabular}}
\end{table}
